Normalization-Equivariant Neural Networks with Application to Image Denoising

In many information processing systems, it may be desirable to ensure that any change of the input, whether by shifting or scaling, results in a corresponding change in the system response. While deep neural networks are gradually replacing all traditional automatic processing methods, they surprisingly do not guarantee such normalization-equivariance (scale + shift) property, which can be detrimental in many applications. To address this issue, we propose a methodology for adapting existing neural networks so that normalization-equivariance holds by design. Our main claim is that not only ordinary convolutional layers, but also all activation functions, including the ReLU (rectified linear unit), which are applied element-wise to the pre-activated neurons, should be completely removed from neural networks and replaced by better conditioned alternatives. To this end, we introduce affine-constrained convolutions and channel-wise sort pooling layers as surrogates and show that these two architectural modifications do preserve normalization-equivariance without loss of performance. Experimental results in image denoising show that normalization-equivariant neural networks, in addition to their better conditioning, also provide much better generalization across noise levels.

==> bib.tex <==
{
\small
\begin{thebibliography}{1}
\setcounter{enumiv}{0}

\bibitem{homogeneous_functions} S. Mohan, Z. Kadkhodaie, E.P. Simoncelli and C. Fernandez-Granda, ``Robust and interpretable blind image denoising via bias-free convolutional neural networks,'' ICLR 2020.

\bibitem{resnet} K. He, X. Zhang, S. Ren, and J. Sun, ``Deep residual learning for image recognition,'' in {\em Proceedings of the IEEE conference on computer vision and pattern recognition}, pp. 770-778, 2016.


\bibitem{batchnorm} S. Ioffe and C. Szegedy, ``Batch normalization: Accelerating deep network training by reducing internal covariate shift,'' in {\em International conference on machine learning}, pmlr, pp. 448-456, 2015.

%\bibitem{instancenorm} D. Ulyanov, A. Vedaldi, and V. Lempitsky, ``Instance normalization: The missing ingredient for fast stylization,'' {\em arXiv preprint arXiv:1607.08022}, 2016.

%\bibitem{groupnorm} Y. Wu and K. He, ``Group normalization,'' in {\em Proceedings of the European conference on computer vision (ECCV)}, pp. 3-19, 2018.

%\bibitem{beyondbatchnorm} E. S. Lubana, R. Dick, and H. Tanaka,  ``Beyond batchnorm: Towards a unified understanding of normalization in deep learning,'' in {\em Advances in Neural Information Processing Systems}, 34, pp. 4778-4791, 2021.


\bibitem{equivariant1} T. S. Cohen, M. Welling, ``Group equivariant convolutional networks,'' in  {\em International Conference on Machine Learning}, pp. 2990–2999, 2016.

\bibitem{equivariant_graph2} N. Keriven and G. Peyré, ``Universal invariant and equivariant graph neural networks,'' in {\em  Advances in Neural Information Processing Systems}, vol. 32, 2019.

\bibitem{equivariant_graph3} V. G. Satorras, E. Hoogeboom, and M. Welling, ``E (n) equivariant graph neural networks,'' in {\em International conference on machine learning} PMLR, pp. 9323-9332, 2021.

\bibitem{equivariant_graph4} S. Batzner, A. Musaelian, L. Sun, \textit{et al.}, ``E (3)-equivariant graph neural networks for data-efficient and accurate interatomic potentials,'' in {\em Nature communications}, vol. 13, no. 1, p. 2453, 2022.


\bibitem{equivariant_image} D. Marcos, M. Volpi, N. Komodakis, and D. Tuia, ``Rotation equivariant vector field networks,'' in {\em Proceedings of the IEEE International Conference on Computer Vision}, pp. 5048-5057, 2017.

\bibitem{equivariant_image2}
M. Weiler, F. A. Hamprecht, and M. Storath, ``Learning steerable filters for rotation equivariant cnns,'' in {\em Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition}, pp. 849-858, 2018.

\bibitem{equivariant_image3}
B. S. Veeling, J. Linmans, J. Winkens, T. Cohen,  and M. Welling, ``Rotation equivariant CNNs for digital pathology,''  in {\em Medical Image Computing and Computer Assisted Intervention–MICCAI: 21st International Conference, Granada, Spain, Proceedings, Part II 11}. Springer International Publishing, pp. 210-218, 2018.

\bibitem{equivariant_image4}
D. K. Gupta, D. Arya, and E. Gavves, ``Rotation equivariant siamese networks for tracking,'' in  {\em Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pp. 12362-12371, 2021.


\bibitem{equivariant_pointcloud1} N. Thomas, T. Smidt, S. Kearnes, L.
Yang, L. Li, K. Kohlhoff, and P. Riley, ``Tensor field networks: Rotation- and translation-equivariant neural networks for 3D point clouds,'' 
{\em arXiv preprint arXiv:1802.08219}, 2018.

\bibitem{equivariant_pointcloud2} F. Fuchs, D. Worrall, V. Fischer, and M. Welling, (2020). ``Se (3)-transformers: 3d roto-translation equivariant attention networks,'' in  {\em Advances in Neural Information Processing Systems}, vol. 33, pp. 1970-1981, 2020.

\bibitem{equivariant_pointcloud3} G. Bökman, F. Kahl, and A. Flinth, ``Zz-net: A universal rotation equivariant architecture for 2d point clouds,'' in {\em Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pp. 10976-10985, 2022.


\bibitem{equivariant_translation1} K. Fukushima,  ``Neocognitron: A self-organizing neural network model for a mechanism of pattern recognition unaffected by shift in position,'' in {\em  Biol. Cybernetics}, vol.36, pp. 193–202,
1980.

\bibitem{equivariant_translation2} Y. LeCun, B. Boser, J. S. Denker, D. Henderson, R. E.
Howard, W. Hubbard, and L. D. Jackel, ``Backpropagation
applied to handwritten zip code recognition,'' in {\em Neural Computation}, vol. 1, no. 4, pp. 541–551, 1989.








\bibitem{convallaria} M. Prakash, M. Lalit, P. Tomancak, A. Krul, and F. Jug, ``Fully unsupervised probabilistic noise2void'' in {\em IEEE 17th International Symposium on Biomedical Imaging (ISBI)}, pp. 154-158, 2020.


%\bibitem{bilateral_filter} C. Tomasi and R. Manduchi, ``Bilateral filtering for gray and color images,'' Sixth International Conference on Computer Vision (IEEE Cat. No.98CH36271), Bombay, India, pp. 839-846, 1998.

\bibitem{TV} L. I. Rudin, S. Osher, and E. Fatemi, ``Nonlinear total variation based noise removal algorithms,'' in {\em Physica D: nonlinear phenomena}, vol. 60, pp. 259-268, 1992.

%\bibitem{dct2net} S. Herbreteau and C. Kervrann, ``DCT2net: An Interpretable Shallow CNN for Image Denoising,'' in {\em IEEE Transactions on Image Processing}, vol. 31, pp. 4292-4305, 2022.

%\bibitem{Anscombe} L. Starck, F. Murtagh, and A. Bijaoui, ``Image Processing and Data Analysis: The Multiscale Approach,'' in {\em Cambridge University Press}, 1998.

\bibitem{DCT} G. Yu and G. Sapiro, ``DCT image denoising:  a simple and effective image denoising algorithm,'' in {\em Image Processing On Line}, vol. 1, pp. 292–296, 2011.


%\bibitem{ksvd} M. Elad and M. Aharon, ``Image denoising via sparse and redundant representations over learned dictionaries,'' in {\em IEEE Transactions on Image Processing}, vol. 15, no. 12, pp. 3736-3745, 2006.

\bibitem{nlmeans} A. Buades, B. Coll, and J.-M. Morel, ``A review of image denoising algorithms, with a new one,'' in {\em SIAM Journal on Multiscale Modeling and Simulation}, vol. 4, no. 2, pp. 490-530, 2005.


\bibitem{nlmeans2} A. Buades, B. Coll, and J.-M. Morel, ``A non-local algorithm for image
denoising,'' in {\em Proc. IEEE Comput. Soc. Conf. Comput. Vis. Pattern
Recognit.}, San Diego, CA, USA, pp. 60–65, 2005.

\bibitem{OWF} Q. Jin, I. Grama, C. Kervrann, and Q. Liu, ``Non-local means and optimal weights for noise removal,'' in {\em SIAM Journal on Imaging Sciences}, vol. 10, no. 4, pp. 1878-1920, 2017.

\bibitem{tv-means} C. Louchet and L. Moisan, ``Total variation as a local filter,'' {\em SIAM Journal on Imaging Sciences}, vol. 4, no. 2, pp. 651-694, 2011.

\bibitem{nlmeans3} J. V. Manjon, J. C. Caballero, J. J. Lull, G. G. Marti, L. M. Bonmati, and M. Robles, ``MRI denoising using non local means,'' in  {\em Med. Image. Anal.},  vol. 12, no. 4, pp. 514-523, 2008.


\bibitem{nlmeans_parameters} V. Duval, J. F. Aujol, and Y. Gousseau, ``On the parameter choice for the non-local means,'' Tech. Rep. HAL-00468856, 2010.



%\bibitem{LIDIA} G. Vaksman, M. Elad, and P. Milanfar, ``LIDIA: Lightweight Learned Image Denoising With Instance Adaptation,'' in {\em Conference on Computer Vision and Pattern Recognition (CVPR) Workshops}, June, 2020.

\bibitem{BM3D} K. Dabov, A. Foi, V. Katkovnik, and K. Egiazarian, ``Image denoising by sparse 3D transform-domain collaborative filtering,'' in {\em IEEE Transactions on Image Processing}, vol. 16, no. 8, pp. 2080–2095, 2007.

%\bibitem{nlbayes} A. Buades, M. Lebrun, and J.-M. Morel, ``A Non-local Bayesian image denoising algorithm,'' in {\em SIAM Journal on Imaging Science}, vol. 6, no. 3, pp. 1665-1688, 2013. 
 

\bibitem{nlridge} S. Herbreteau and C. Kervrann, ``Towards a Unified View of Unsupervised Non-Local Methods for Image Denoising: The NL-Ridge Approach,'' in {\em 2022 IEEE International Conference on Image Processing (ICIP)}, pp. 3376-3380, Bordeaux, France, 2022. 

%\bibitem{lichi} S. Herbreteau and C. Kervrann, ``Unsupervised Linear and Iterative Combinations of Patches for Image Denoising'', arXiv preprint arXiv:2212.00422, 2022.


\bibitem{WNNM} S. Gu, L. Zhang, W. Zuo, and X. Feng, ``Weighted Nuclear Norm Minimization with Application to Image Denoising,'' in {\em IEEE Conference on Computer Vision and Pattern Recognition}, Columbus, OH, USA, 2014, pp. 2862-2869.


%\bibitem{SAIST} W. Dong, G. Shi, and X. Li, ``Nonlocal image restoration with bilateral variance estimation: a low-rank approach,'' in {\em IEEE Transactions on Image Processing}, vol. 22, no. 2, pp. 700–711, 2013.

%\bibitem{LSSC} J. Mairal, F. Bach, J. Ponce, G. Sapiro, and A. Zisserman, ``Non-local sparse models for image restoration,'' in {\em IEEE 12th International Conference on Computer Vision}, Tokyo, Japan, 2009, pp. 2272-2279.

%\bibitem{NCSR} W. Dong, L. Zhang, G. Shi, and X. Li, ``Nonlocally Centralized Sparse Representation for Image Restoration,'' in {\em IEEE Transactions on Image Processing}, vol. 22, no. 4, pp. 1620-1630, 2013.

%\bibitem{EPLL} D. Zoran and Y. Weiss, ``From learning models of natural image patches to whole image restoration,'' in {\em 2011 International Conference on Computer Vision}, pp. 479-486, 2011.
 

%\bibitem{PEWA} C. Kervrann, ``PEWA : Patch-based exponentially weighted aggregation for image denoising,'' in {\em Neural Information Processing Systems}, Montreal, Canada, 2014, pp. 2150–2158.


%\bibitem{optimalS} C. Kervrann and J. Boulanger, ``Optimal spatial adaptation for patch-based image denoising,'' in {\em IEEE Transactions on Image Processing}, vol. 15, no. 10, pp. 2866-2878, 2006.

%\bibitem{localA} C. Kervrann and J. Boulanger, ``Local adaptivity to variable smoothness for exemplar-based image denoising and representation,'' in {\em International Journal of Computer Vision}, vol. 79, no. 1, pp. 45-69, 2008.

\bibitem{dncnn} K. Zhang, W. Zuo, Y. Chen, D. Meng, and L. Zhang, ``Beyond a gaussian denoiser: residual learning of deep CNN for image denoising,'' in {\em IEEE Transactions on Image Processing}, vol. 26, no. 7, pp. 3142–3155, 2017.

\bibitem{ffdnet} K. Zhang, W. Zuo, and L. Zhang, ``FFDNet: Toward a Fast and Flexible Solution for {CNN} based Image Denoising,'' in {\em IEEE Transactions on Image Processing}, vol. 27, no. 9, pp. 4608–4622, 2018.

\bibitem{drunet}  K. Zhang, Y. Li, W. Zuo, L. Zhang, L. Van Gool, and R. Timofte, ``Plug-and-play image restoration with deep denoiser prior,'' in {\em IEEE Transactions on Pattern Analysis and Machine Intelligence}, 2021.


%\bibitem{rnan} Y. Zhang, K. Li, K. Li, B. Zhong, and Y. Fu, ``Residual non-local attention networks for image restoration,'' in {\em International Conference on Learning Representations (ICLR)}, May 2019.

\bibitem{red30} X. Mao, C. Shen, and Y. Yang. ``Image restoration using very deep convolutional encoder-decoder networks with symmetric skip connections,'' in {\em Advances in Neural Information Processing Systems}, pp. 2802–2810, 2016.

\bibitem{tnrd} Y. Chen and T. Pock, ``Trainable nonlinear reaction diffusion: A flexible framework for fast and effective image restoration,'' in {\em IEEE Transactions on Pattern Analysis and Machine Intelligence}, vol. 39, no. 6, pp. 1256–1272, 2017.

\bibitem{nlrn} Ding Liu, Bihan Wen, Yuchen Fan, Chen Change Loy, and Thomas S Huang, ``Non-local recurrent network for image restoration,'' in {\em Advances in Neural Information Processing Systems}, pp. 1673–1682, 2018.

%\bibitem{n3net} P. Tobias and R. Stefan, ``Neural Nearest Neighbors Networks,''  in {\em Advances in Neural Information Processing Systems (NeurIPS)}, 2018.

\bibitem{swinir} J. Liang, J. Cao, G. Sun, K. Zhang, L.
Van Gool, and R. Timofte. ''Swinir: Image restoration using swin transformer,'' in {\em IEEE International Conference on
Computer Vision Workshops}, pp. 1833–1844, 2021.

%\bibitem{mlp} H. C. Burger, C. J. Schuler, and S. Harmeling, ``Image denoising: Can plain  neural  networks  compete  with  BM3D?,'' in {\em IEEE  Conference  on Computer Vision and Pattern Recognition}, pp. 2392–2399, 2012.

%\bibitem{DIP}  D. Ulyanov, A. Vedaldi, and V. Lempitsky, ``Deep image prior,'' in {\em Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition}, pp. 9446–9454, 2018.

%\bibitem{DND} T. Plotz and S. Roth, ``Benchmarking denoising algorithms with real photographs,'' in {\em IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, July 2017.

\bibitem{berkeley} D.  Martin,  C.  Fowlkes,  D.  Tal,  and  J.  Malik, ``A  database  of  human segmented natural images and its application to evaluating segmentation algorithms and measuring ecological statistics,'' in {\em International Conference on Computer Vision}, vol. 2, pp. 416–423, 2001.

%\bibitem{urban} J.-B. Huang,  A. Singh, and N. Ahuja, ``Single image super-resolution from transformed self-exemplars,'' in {\em Conference on Computer Vision and Pattern Recognition (CVPR)}, pp.5197–5206, 2015.

%\bibitem{adam} D. Kingma and J. Ba, ``Adam: A method for stochastic optimization,'' in {\em International Conference for Learning Representations}, 2015.




\end{thebibliography}
}

==> instructions.tex <==

\section{Submission of papers to NeurIPS 2023}


Please read the instructions below carefully and follow them faithfully. \textbf{Important:} This year the checklist will be submitted separately from the main paper in OpenReview, please review it well ahead of the submission deadline: \url{https://neurips.cc/public/guides/PaperChecklist}.


\subsection{Style}


Papers to be submitted to NeurIPS 2023 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2023 are the same as those in previous years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the website at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2023.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2023 is \verb+neurips_2023.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit, as long as you do not say which conference it was submitted to. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS. 


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2023.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.


\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2023+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2023}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous'' and include a copy of the anonymized paper in the supplementary material.


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Math}
Note that display math in bare TeX commands will not create correct line numbers for submission. Please use LaTeX (or AMSTeX) commands for unnumbered display math. (You really shouldn't be using \$\$ anyway; see \url{https://tex.stackexchange.com/questions/503/why-is-preferable-to} and \url{https://tex.stackexchange.com/questions/40492/what-are-the-differences-between-align-equation-and-displaymath} for more information.)

\subsection{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2023/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}



\section{Supplementary Material}

Authors may wish to optionally include extra information (complete proofs, additional experiments and plots) in the appendix. All such materials should be part of the supplemental material (submitted separately) and should NOT be included in the main submission.


\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tableau.tex <==
\renewcommand{\arraystretch}{1.1}
\begin{table*}[!t]
\centering
\caption{The PSNR (dB) results of different deep-learning-based methods applied to three datasets corrupted with synthetic white Gaussian noise and $\sigma=15$, $25$ and $50$.}

\resizebox{\columnwidth}{!}{%
  \begin{NiceTabular}{c@{\hspace{0.1cm}}  c@{\hspace{0.5cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}}  c@{\hspace{0.7cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.7cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.0cm}} c}
  \hline
 &  Dataset  & \multicolumn{5}{c}{Set12} & \multicolumn{5}{c}{BSD68} & \multicolumn{5}{c}{Urban100} & \\\hline\hline\noalign{\vskip 0.1cm}

   \multicolumn{2}{c}{ Noise level $\sigma$} &  15 &/& 25  &/& 50 &  15 &/& 25  &/& 50 &   15 &/& 25  &/& 50 & \\[0.1cm]
   \hline\noalign{\vskip 0.1cm}

 \multirow{3}{*}{\rotatebox[origin=c]{70}{\small \textit{\textbf{DRUNet}}}} & \textit{ordinary}   &   - &/& -  &/& - &   - &/& -  &/& - &  -  &/& - &/&   -  &\\
 & \textit{scale-equiv}  &   33.25 &/& 30.94  &/& 27.90 &   31.91 &/& 29.48  &/& 26.59 &  33.44  &/& 31.11  &/& 27.96  &\\
 & \textit{norm-equiv}  &   33.16 &/& 30.87  &/& 27.82 &   31.87 &/& 29.44  &/& 26.54 &   33.17  &/& - &/&   -  &\\
 


\cdashline{1-18}\noalign{\vskip 0.1cm}
%\hline\noalign{\vskip 0.1cm}

   \multirow{3}{*}{ \rotatebox[origin=c]{70}{\small \textit{\textbf{FDnCNN}}}} & \textit{ordinary}  &   - &/& -  &/& - &   31.69 &/& 29.22  &/& 26.27 &  -  &/& - &/&   -  &\\
 & \textit{scale-equiv}  &   - &/& -  &/& - &   - &/& -  &/& - &  -  &/& - &/&   - &\\
 & \textit{norm-equiv}  &   - &/& -  &/& - &   - &/& -  &/& - &  -  &/& - &/&   -  & \\[0.1cm] \hline
\end{NiceTabular}%
}

\label{resultsPSNR}
\end{table*}



==> tableau_color.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[!t]
\centering
\caption{The PSNR (dB) results of different methods applied to three datasets corrupted with synthetic white Gaussian noise and $\sigma=15$, $25$ and $50$. * means a color dataset.}

\resizebox{\columnwidth}{!}{%
  \begin{NiceTabular}{|c@{\hspace{0.1cm}}  c@{\hspace{0.5cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}}  c@{\hspace{0.7cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.7cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.7cm}}
c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.08cm}} c@{\hspace{0.0cm}} c|}
  \hline
 &    & \multicolumn{5}{c}{Set12} & \multicolumn{5}{c}{BSD68} & \multicolumn{5}{c}{Set5*} & \multicolumn{5}{c}{CBSD68*} & \\\hline\hline\noalign{\vskip 0.1cm}

   \multicolumn{2}{c}{ Noise level $\sigma$} &  15 &/& 25  &/& 50 &  15 &/& 25  &/& 50 &   15 &/& 25  &/& 50 &   15 &/& 25  &/& 50 & \\[0.1cm]
   \hline\noalign{\vskip 0.1cm}

 \multirow{3}{*}{\rotatebox[origin=c]{70}{\small \textit{\textbf{DRUnet}}}} & \textit{ordinary}   &   - &/& -  &/& - &   - &/& -  &/& - &  -  &/& - &/&   - &  -  &/& - &/&   - &\\
 & \textit{scale-equiv}  &   33.25 &/& 30.94  &/& 27.90 &   31.91 &/& 29.48  &/& 26.59 &  -  &/& - &/&   29.80 &  34.30  &/& 31.69 &/&  28.51 &\\
 & \textit{norm-equiv}  &   33.16 &/& 30.87  &/& 27.82 &   31.87 &/& 29.44  &/& 26.54 &  -  &/& - &/&   - &  -  &/& - &/&   - &\\
 


\cdashline{1-23}\noalign{\vskip 0.1cm}
%\hline\noalign{\vskip 0.1cm}

   \multirow{3}{*}{ \rotatebox[origin=c]{70}{\small \textit{\textbf{FDnCNN}}}} & \textit{ordinary}  &   - &/& -  &/& - &   31.69 &/& 29.22  &/& 26.27 &  -  &/& - &/&   - &  -  &/& - &/&   - &\\
 & \textit{scale-equiv}  &   - &/& -  &/& - &   - &/& -  &/& - &  -  &/& - &/&   - &  -  &/& - &/&   - &\\
 & \textit{norm-equiv}  &   - &/& -  &/& - &   - &/& -  &/& - &  -  &/& - &/&   - &  -  &/& - &/&   - & \\[0.1cm] \hline
\end{NiceTabular}%
}

\label{resultsPSNR}
\end{table*}


